Subjective assessment of the impact of a content adaptive optimiser for compressing 4K HDR content with AV1

Since 2015 video dimensionality has expanded to higher spatial and temporal resolutions and a wider colour gamut. This High Dynamic Range (HDR) content has gained traction in the consumer space as it delivers an enhanced quality of experience. At the same time, the complexity of codecs is growing. This has driven the development of tools for content-adaptive optimisation that achieve optimal rate-distortion performance for HDR video at 4K resolution. While improvements of just a few percentage points in BD-Rate (1-5\%) are significant for the streaming media industry, the impact on subjective quality has been less studied especially for HDR/AV1. In this paper, we conduct a subjective quality assessment (42 subjects) of 4K HDR content with a per-clip optimisation strategy. We correlate these subjective scores with existing popular objective metrics used in standard development and show that some perceptual metrics correlate surprisingly well even though they are not tuned for HDR. We find that the DSQCS protocol is too insensitive to categorically compare the methods but the data allows us to make recommendations about the use of experts vs non-experts in HDR studies, and explain the subjective impact of film grain in HDR content under compression.

==> backup.tex <==

\begin{figure}[]
\centering
\begin{subfigure}{.5\columnwidth}
\centering
\includegraphics[width=\columnwidth]{images/corr/pearson-mos-all.png}
\caption{All-MOS}
\label{fig:sub1}
\end{subfigure}%
\begin{subfigure}{.5\columnwidth}
\centering
\includegraphics[width=\columnwidth]{images/corr/pearson-dmos-all.png}
\caption{All-DMOS}
\label{fig:sub2}
\end{subfigure}\\[2ex]
\begin{subfigure}{0.5\columnwidth}
\centering
\includegraphics[width=\columnwidth]{images/corr/pearson-dmos-noexperts.png}
\caption{Non-Experts DMOS}
\label{fig:sub3}
\end{subfigure}%
\begin{subfigure}{0.5\columnwidth}
\centering
\includegraphics[width=0.93\columnwidth, height=\columnwidth]{images/corr/pearson-dmos-experts.png}
\caption{Experts DMOS}
\label{fig:sub3}
\end{subfigure}
\caption{Pearson Correlation between different metrics.}
\label{fig:corr_heat}
\end{figure}




% \begin{table}[h]
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{@{}ccccccc@{}}
% \toprule
% \multirow{2}{*}{\textbf{Clip}} & \multicolumn{3}{c}{\textbf{BD-Rate (\%)}} & \multicolumn{3}{c}{\textbf{BD-MOS}} \\ \cmidrule(l){2-7} 
%  & \textbf{MOS} & \textbf{MOS-P910} & \textbf{MOS-P913} & \textbf{MOS} & \textbf{MOS-P910} & \textbf{MOS-P913} \\ \midrule
% MeridanFace & -12.485 & -3.590 & -13.679 & 2.676 & 0.918 & 1.485 \\
% NocturneRoom & -47.633 & -22.210 & -48.463 & 0.667 & 0.929 & 0.731 \\
% SVTSmithyHouse & 35.727 & 29.804 & 36.558 & 1.317 & 1.553 & 1.180 \\
% CablesButterfly & 40.684 & 30.595 & 36.154 & 0.934 & 0.656 & 0.902 \\
% CosmosRunningSheep & -2.234 & -2.404 & -2.544 & -2.961 & -1.732 & -2.601 \\
% SolLevanteFireDragon & -3.152 & -1.316 & -1.268 & -1.913 & -0.853 & -2.414 \\ \midrule
% \textit{\textbf{Average}} & 1.818 & 5.147 & 1.126 & 0.120 & 0.245 & -0.119 \\ \bottomrule
% \end{tabular}%
% }
% \caption{BD-rate (\%) savings measured for points after removing outlier points in the RD-Curve which are non-monotonic, \textit{negative} is better. The BD-MOS was measured on the full RD-curve without any modifications, \textit{positive} is better.}
% \label{tab:mos-table}
% \end{table}


%\begin{figure}[h]
%    \begin{tikzpicture}
%    \centering
%    \node[anchor=south west,inner sep=0] (image) at (0,0) {\includegraphics[width=\columnwidth]{images/NocturneRoomAV1.png}}; \begin{scope}
%    \node[draw=none, anchor=south west, text=red!60!white, inner sep=0, font=\sffamily] at (0.1,0.1){\small $qp27$};
%    \node[draw=none, anchor=south west, text=red!60!white, inner sep=0, font=\sffamily] at (3.5,0.1){\small $68.36$};
%    \node[draw=none, anchor=south west, text=red!60!white, inner sep=0, font=\sffamily] at (4.5,0.1){\small $qp49$};
%    \node[draw=none, anchor=south west, text=red!60!white, inner sep=0, font=\sffamily] at (7.75,0.1){\small $68.70$};
%    \node[draw=none, anchor=south west, text=red!60!white, inner sep=0, font=\sffamily] at (0.1,4.5){\small $45Mb/s$};
%    \node[draw=none, anchor=south west, text=red!60!white, inner sep=0, font=\sffamily] at (4.5,4.5){\small $2.7Mb/s$};
%    
%    \end{scope}\end{tikzpicture}    
%    \caption{A crop of a frame of NocturneRoom sequence at two $qp$ (left: $qp$27, right:$qp$49). The perceived quality in terms of MOS score is approximately the same between both ($\Delta0.34$) while both exhibit different levels of noise detail. }
%    \label{fig:noctroomnoise}
%\end{figure}
%subjective RDCurves, P910/913 normalisation parts etc

%Things to write down 
%a) QP selection should be very careful and we should align the bitrate so we can do statistical analysis (for reducing variance). Either matching non-opt video's Bitrate with opt video's bitrate. 
%a.1) ACK Opinion needed: We can do something like 12 QPs and find the values which can have target quality.
%
%b) The DSCQS protocol may not be optimal for doing a study with two techniques involving not-so-significant quality difference, we may need to go side-by-side pairwise comparison, with an option for subjects to revisit the video playback before making a decision. 
%c) Choice of videos should be careful,
%c.1) Noise in the source sequences causes issues, which is not visible in the current objective metrics. 
%c.2) How representative is that for real-world, good for testing sets.
%c.3) Framerates of videos are different at 24,50, 59.94, 60, we might stick to one framerate for the whole study. To avoid confusion of perception
%c.4) 

%For the study, we have in total of 2016 data points (6 videos $\times$ 4 $qp$ $\times$ 2 modes $\times$ 42 subjects), and we have 1008 ratings for both baseline (A) and optimised method (B) in which 434 times people preferred optimised method over non-optimised. Further investigating we found that people preferred B over A with more than 5, 10, 20, and 30 DMOS scores for 265, 166, 68, and 33 times respectively, and 102 times people said A is equal to B. In total, 432 times subjects preferred compressed video over the source video. The preference in terms of MOS scores is also similar in range. 
% DMOS: 265, 166, 68, 33 for DMOS, and 102 times equal 
% MOS 275, 152, 59 and 22


%Figure ~\ref{fig:noctroomnoise} showcases a zoomed-in view of a patch of a sequence which is dark and has noise, where MOS score for $qp27$ (~45Mb/s) and $qp49$ (2.7Mb/s) have very similar MOS score (~68). The noise and detail are different in both, the $qp27$ video retains noise from the source, and the latter ($qp49$) introduces compression artefacts (Blurriness and loss of details), which was subjectively similar for non-experts. 

%RD curves areTabe ~\ref{tab:mos-table} reports subjective improvements in terms of BD-Rate(\%) and BD-MOS for MOS, MOS-P910, and MOS-P913. The BD rate (\%) is computed after removing outlier points which are not monotonic (4 clips with 3 points). BD-MOS is computed on 4 points without any outlier rejection.




%\begin{figure*}[]
% \centering
%  \begin{subfigure}[b]{0.20\textwidth}
%    \centering
%    \includegraphics[width=\textwidth]{images/mos-all/NocturneRoom_3840x2160_60fps_hdr10_R0.y4m-p910.png}
%    \caption{NocturneRoom}
%    \label{fig:p913-mos-all-noctRoom}
%  \end{subfigure}
%  \hspace*{0.01\textwidth}
%  \begin{subfigure}[b]{0.20\textwidth}
%    \centering
%    \includegraphics[width=\textwidth]{images/mos-all/aomcosmos_3840x2160_24_hdr10_11589-11752_R0.y4m-p910.png}
%    \caption{CosmosRunningSheep}
%    \label{fig:p913-mos-all-cosmos}
%  \end{subfigure}
%  \hspace*{0.01\textwidth}
%  \begin{subfigure}[b]{0.20\textwidth}
%    \centering
%    \includegraphics[width=\textwidth]{images/mos-all/wipe_3840x2160_5994_10bit_420_8750-9050_R0.y4m-p910.png}
%    \caption{CablesButteryfly}
%    \label{fig:p913-mos-wipe}
%  \end{subfigure}
%  \hspace*{0.01\textwidth}
%  \begin{subfigure}[b]{0.20\textwidth}
%    \centering
%    \includegraphics[width=\textwidth]{images/mos-all/aomsol_levante_3840x2160_24_hdr10_2268-2412_R0.y4m-p910.png}
%    \caption{SolLevanteFireDragon}
%    \label{fig:p913-mos-all-solevante}
%  \end{subfigure}
%  \hspace*{0.01\textwidth}
%  \begin{subfigure}[b]{0.20\textwidth}
%    \centering
%    \includegraphics[width=\textwidth]{images/mos-all/svtsmithy_3840x2160_50_10bit_420p_R0.y4m-p910.png}
%    \caption{SVTSmithyHouse}
%    \label{fig:p913-mos-svt}
%  \end{subfigure}
%  \hspace*{0.01\textwidth}
%  \begin{subfigure}[b]{0.20\textwidth}
%    \centering
%    \includegraphics[width=\textwidth]{images/mos-all/aommeridian1_3840x2160_5994_hdr10_15932-16309_R0.y4m-p910.png}
%    \caption{MeridianFace}
%    \label{fig:p913-mos-all-merid}
%  \end{subfigure}
%  \hspace*{0.01\textwidth}
%  \begin{subfigure}[b]{0.20\textwidth}
%    \centering
%    \includegraphics[width=\textwidth]{images/mos-experts-v2/aommeridian1_3840x2160_5994_hdr10_15932-16309_R0.y4m-p910.png}
%    \caption{MeridianFace Expts}
%    \label{fig:p913-mos-expt-merid}
%  \end{subfigure}
%  \hspace*{0.01\textwidth}
%  \begin{subfigure}[b]{0.20\textwidth}
%    \centering
%%aommeridian1_3840x2160_5994_hdr10_15932-16309_R0.y4m-p910.png
%    \includegraphics[width=\textwidth]{images/mos-noexperts/aommeridian1_3840x2160_5994_hdr10_15932-16309_R0.y4m-p910.png}
%    \caption{MeridianFace N-Expts}
%    \label{fig:p913-mos-noexpt-merid}
%  \end{subfigure}
%    %    \hfill 
%  \vspace{-.5em}
%  \caption{Fig~\ref{fig:p913-mos-all-noctRoom}-\ref{fig:p913-mos-all-merid}: P910-MOS Score variation for all the 42 subjects who participated in the study, Fig~\ref{fig:p913-mos-expt-merid} and Fig~\ref{fig:p913-mos-noexpt-merid} denotes P910-MOS scores for the Merdian sequence for the subjects who are experts (10) and non-experts (32) respectively. }% as shown in Table \ref{tab:average-table}}
%    \vspace{-1em}
% 
%  \label{fig:mos-scores}
%\end{figure*}



\begin{figure*}[]
 \centering
  \begin{subfigure}[b]{0.22\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/dmos-all/NocturneRoom_3840x2160_60fps_hdr10_R0.y4m-p910.png}
    \caption{NocturneRoom}
  \end{subfigure}
  \hspace*{0.01\textwidth}
  \begin{subfigure}[b]{0.22\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/dmos-all/aomcosmos_3840x2160_24_hdr10_11589-11752_R0.y4m-p910.png}
    \caption{Cosmos}
  \end{subfigure}
  \hspace*{0.01\textwidth}
  \begin{subfigure}[b]{0.22\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/dmos-all/wipe_3840x2160_5994_10bit_420_8750-9050_R0.y4m-p910.png}
    \caption{Wipe}
  \end{subfigure}
  \hspace*{0.01\textwidth}
  \begin{subfigure}[b]{0.22\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/dmos-all/aomsol_levante_3840x2160_24_hdr10_2268-2412_R0.y4m-p910.png}
    \caption{Sol Levante}
  \end{subfigure}
  \hspace*{0.01\textwidth}
  \begin{subfigure}[b]{0.22\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/dmos-all/svtsmithy_3840x2160_50_10bit_420p_R0.y4m-p910.png}
    \caption{SVT Smithy}
  \end{subfigure}
  \hspace*{0.01\textwidth}
  \begin{subfigure}[b]{0.22\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/dmos-all/aommeridian1_3840x2160_5994_hdr10_15932-16309_R0.y4m-p910.png}
    \caption{Meridian}
  \end{subfigure}
  \hspace*{0.01\textwidth}
  \begin{subfigure}[b]{0.22\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/dmos-experts/aommeridian1_3840x2160_5994_hdr10_15932-16309_R0.y4m-p910.png}
    \caption{Meridian Experts}
  \end{subfigure}
  \hspace*{0.01\textwidth}
  \begin{subfigure}[b]{0.22\textwidth}
    \centering
    %aommeridian1_3840x2160_5994_hdr10_15932-16309_R0.y4m-p910.png
    \includegraphics[width=\textwidth]{images/dmos-noexperts/aommeridian1_3840x2160_5994_hdr10_15932-16309_R0.y4m-p910.png}
    \caption{Meridian No-Experts}
  \end{subfigure}

  %    \hfill 
  \vspace{-.5em}
  %\caption{Fig~\ref{fig:p913-mos-all-noctRoom}-\ref{fig:p913-mos-all-merid}: P910-MOS Score variation for all the 42 subjects who participated in the study, Fig~\ref{fig:p913-mos-expt-merid} and Fig~\ref{fig:p913-mos-noexpt-merid} denotes P910-MOS scores for the Merdian sequence for the subjects who are experts (10) and non-experts (32) respectively. }% as shown in Table \ref{tab:average-table}}
 % \label{fig:mos-scores}
\end{figure*}
